Efficient Multiway Hash Join on Reconfigurable Hardware

We propose the algorithms for performing multiway joins using a new type of coarse grain reconfigurable hardware accelerator~-- ``Plasticine''~-- that, compared with other accelerators, emphasizes high compute capability and high on-chip communication bandwidth. Joining three or more relations in a single step, i.e. multiway join, is efficient when the join of any two relations yields too large an intermediate relation. We show at least 200X speedup for a sequence of binary hash joins execution on Plasticine over CPU. We further show that in some realistic cases, a Plasticine-like accelerator can make 3-way joins more efficient than a cascade of binary hash joins on the same hardware, by a factor of up to 45X.

==> formal-algo.tex <==
\begin{algorithm}
 \KwData{Large size relations K(C1,C2). Hash function H and G are used to for hashing values of columns C1 and C2 respectively}
 \KwResult{ Number of partitions for K as \#Kpart. Partitions Ki(C1,C2) of K}
 $i \leftarrow 0$\;
\While{(All records of K are not hashed on B and C)}{
        If H is NOT Null then $h_{b} \leftarrow H(k.b)$ else $h_{b}=0$\;
        If G is not Null then $g_{c} \leftarrow G(k.c)$ else $g_{c}=0$\ ;
        $Ki[h_{b}][g_{c}] \leftarrow k(b,c)$\;
        $i \leftarrow i+1$\;
    }
    $ \#Kpart \leftarrow i$\;
    Return (\#Kpart, Ki(C1,C2))\;
 \caption{Pseudo-code for partitioning large relation K(C1,C2)}
 %, and \# introduces a comment. 
 \label{algo:partition}
\end{algorithm}

\begin{algorithm}
 \KwData{Relations R(A,B), S(B,C) and T(C, D). Hardware has $N^2$ memory grid. Column B values hashed using $h()$ to 1 to N values. Column C hashed using $g()$ to 1 to N values.}
 \KwResult{Tuples from T1, T2 and T3 joined on common values of B and C.}
 $Ti \leftarrow Partition(T(C,D), G,0) [\#Tpart]$\;
 $Si \leftarrow Partition(S(B,C), H,G) [\#Spart]$ (Si partitions are ordered on Hb values) \;
 $Ri \leftarrow Partition(R(A,B), 0,H) [\#Rpart]$\;
\For{All partitions Ri of R}{
\While{(All records of Ri are not hashed on B)}{
    $h_{b} \leftarrow h(ri.b)$\;
    $MemGrid[h_{b}][*] \leftarrow ri(*,b)$\;
    }
\For{All partitions Ti of T}{
\While{(All records of Ti are not hashed on C)}{
    $g_{c} \leftarrow g(ti.c)$\;
    $MemGrid[*][g_{c}] \leftarrow ti(c,*)$\;
    }  
  \While{(All records of Si are not hashed on B and C)}{
        $h_{b} \leftarrow h(si.b)$\;
        $g_{c} \leftarrow g(si.c)$\;
        $MemGrid[h_{b}][g_{c}] \leftarrow si(b,c)$\;
        Join tuples on B and C in JCU, and Output\;
        Discard Tuples of Si\;
  } % all records meets
  Discard Tuples of Ti\;
  } % all partitions of T
  Discard Tuples of Ri\;
 } % all partitions for R
  \caption{Pseudo-code for First approach of 3-way Linear Join on columns B and C: R(AB), S(BC),T(CD)}
 \label{algo:linearjoin1}
\end{algorithm}

\begin{algorithm}
 \KwData{Relations R(A,B), S(B,C) and T(C, D). Hardware has $N^2$ memory units. Column B values in a partition are hashed using $h()$ to 1 to $N^2$ values. Column C hashed using $g()$.}
 \KwResult{Tuples from R,S  and T joined on common values of B and C.}
 %\textbf{For all partitions T2}\\
 $Ti \leftarrow Partition(T(C,D), g,0) [\#Tpart]$\;
 $Sij \leftarrow Partition(S(B,C),H,g) [\#Spart]$\;
 $Ri \leftarrow Partition(R(A,B), 0, H) [\#Rpart]$\;
\For{Each partition Ri of R till \#Rpart}{\
 \For{All records of Ri}{\
  $h_{b} \leftarrow h(ri.b)$\;
  $MemGrid[h_{b}] \leftarrow ri(*,b)$\;
  } %records of Ri partition
  \For{Each partition Si of S for i as $H_{b}$ till \#Spart}{\
     %$Sij \leftarrow Partition(Si(B,C), 0, g)$\;
     \For{Each partition Sij for j as $g_{c}$ till \#Sipart}{\
       \For{All records of Sij}{
        $h_{b} \leftarrow h(sij.b)$\;
        $MemGrid[h_{b}] \leftarrow sij(b,c)$\;
        } % all records of Sij
       $MemGrid[*]  \leftarrow tj(c,*)$ [broadcast, send to all mem where Sij was sent]\;
       Join tuple from Ri, Sij and Tj\;
       Discard tuples from Sij and Tj\;
     } % all partitions Sij
  }% all partitions of S
  Discard tuples of Ri
} % all partitions of R
 \caption{Pseudo-code for 3-way Linear Join on columns B and C: $R(AB)\bowtie S(BC)\bowtie T(CD)$}.
 \label{algo:linearjoin2}
\end{algorithm}

\begin{algorithm}
{
\KwData{Relations R(A,B), S(B,C) and T(C, A). Assume R, S and T are sufficiently small of sizes that the following can be carried out using only PMUs. Hardware has NXN memory grid. Column A values hashed using $h()$ to 1 to N values. Column B hashed using $g()$ to 1 to N values and Column C hashed using $k()$ to large values.}
\KwResult{Tuples from T1, T2 and T3 joined on common values of A, B and C.}
 %\textbf{For all partitions T2}\\
\While{(All records of T1 are not hashed on A and B)}{
    $h_{a} \leftarrow h(t1.a)$\;
    $g_{b} \leftarrow h(t1.b)$\
    $MemGrid[h_{a}][g_{b}] \leftarrow t1(a,b)$\;
    }
\For{each $k_{c}$ bucket}{
\While{(All records of $T3_{bkt}[k_{c}]$) not hashed on A}{
    $h_{a} \leftarrow h(t3.a)$\;
    $MemGrid[h_{a}][*] \leftarrow t3(*,a)$\;
    }  
\While{(All records of $T2_{bkt}[k_{c}]$ not hashed on B)}{
        $g_{b} \leftarrow g(t2.b)$\;
        $MemGrid[*][g_{b}] \leftarrow t2(b,*)$\;
        }
 \For{all cells in $MemGrid[*][*]$}{
        Join tuples on A, B and C and Output\\
  }
 }
}
\caption{Pseudo-code for 3-way Cyclic Join on columns A, B and C: T1(AB), T2(BC),T3(CA)}
 \label{algo:cyclicjoin}
\end{algorithm}


==> packages.tex <==

%\usepackage{cite}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}

\usepackage{algorithmic}
\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{siunitx} 

\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{textcomp}
\usepackage{epsfig}

\usepackage{comment} 

\usepackage{url}
\usepackage{hyperref}

\usepackage{microtype}
\usepackage{booktabs} % for professional tables

\usepackage{times}
\usepackage{shortcuts_js}

\usepackage{cleveref} 
%\usepackage{authblk}
